Byzantine-Resilient Secure Federated Learning

Secure federated learning is a privacy-preserving framework to improve machine learning models by training over large volumes of data collected by mobile users. This is achieved through an iterative process where, at each iteration, users update a global model using their local datasets. Each user then masks its local model via random keys, and the masked models are aggregated at a central server to compute the global model for the next iteration. As the local models are protected by random masks, the server cannot observe their true values. This presents a major challenge for the resilience of the model against adversarial (Byzantine) users, who can manipulate the global model by modifying their local models or datasets. Towards addressing this challenge, this paper presents the first single-server Byzantine-resilient secure aggregation framework (BREA) for secure federated learning. BREA is based on an integrated stochastic quantization, verifiable outlier detection, and secure model aggregation approach to guarantee Byzantine-resilience, privacy, and convergence simultaneously. We provide theoretical convergence and privacy guarantees and characterize the fundamental trade-offs in terms of the network size, user dropouts, and privacy protection. Our experiments demonstrate convergence in the presence of Byzantine users, and comparable accuracy to conventional federated learning benchmarks.

==> algorithm_general.tex <==
Having all above steps, the overall {\byz} framework can now be presented in Algorithm \ref{Alg_gene}.

\begin{algorithm}[t!]
% \footnotesize
% \small
  \caption{Byzantine-Resilient Secure Aggregation ({\byz})}\label{Alg_gene} 
  \begin{algorithmic}[1]
    \INPUT{Local dataset $\mathcal{D}_i$ of users $i\in[N]$, number of iterations $J$.} \
    \OUTPUT{Global model $(\mathbf{w}^{(J)})$.} \ 
    \vspace{0.1cm} 
    \FOR{iteration $t=0,\ldots,J-1$}
        \FOR{user $i=1,\ldots,N$}
            \STATE Download the global model ${\mathbf{w}}^{(t)}$ from the server.
            
            \STATE Create a local update ${\mathbf{w}}_{i}^{(t)}$ from \eqref{eq:local_model}. 
            
            \STATE Create the quantized model $\overline{\mathbf{w}}_i = \phi(q\cdot Q_q({\mathbf{w}}_i))$ from \eqref{eq:def_w_bar}.
            
            \STATE Generate secret shares $\{\mathbf{s}_{ij}\}_{j\in[N]}$ from \eqref{eq:VSS_def} and send  $\mathbf{s}_{ij}$ to user $j\in[N]$.
            \STATE Generate commitments $\{\mathbf{c}_{ij}\}_{j\in[T]}$ from \eqref{eq:def:commitment} and broadcast $\{\mathbf{c}_{ij}\}_{j\in[T]}$ to all users.
            
            \STATE Verify the secret shares $\{\mathbf{s}_{ji}\}_{j\in[N]}$ by testing \eqref{eq:VSStest}.
            
            \STATE Compute $\{d^{(i)}_{jk}\}_{j,k\in[N]}$ from \eqref{eq:dist} and send the results to the server.
        
            % \vspace{0.1cm}\IF{$l=1$} 
            
            % \STATE Initialize  $\widetilde{\mathbf{s}}_i^{(1)}=\bar{\mathbf{s}}_i^{(1)} = \mathbf{0}$. 
            % \ELSE
            % \STATE Reconstruct the missing values in  $\{\widetilde{\mathbf{s}}_k^{(l-1)}\}_{k\in[N_{l-1}]}$ due to the dropped users in group $l-1$. 
            % \STATE Update the aggregate value $\widetilde{\mathbf{s}}_i^{(l)}$ from  \eqref{eq:sum_rx_data}. 
            % \STATE Compute the coded aggregate value $\bar{\mathbf{s}}_i^{(l)}$ from  \eqref{eq:sum_codedmodel}.     
            % \ENDIF
            % \STATE Send $\{\widetilde{\mathbf{x}}_{i,j}^{(l)},\! \bar{\mathbf{x}}_{i,j}^{(l)}, \! \widetilde{\mathbf{s}}_i^{(l)}\!\!, \bar{\mathbf{s}}_i^{(l)}\}$ to user $j\in[N_{l\!+\!1}]$ in group $l\!+\!1$ ($j\in[N_{final}]$ if $l=L$).   
        \ENDFOR
    
        \STATE Server recovers   $\{\overline{d}_{jk}\}_{j,k\in[N]}$ in \eqref{eq:distance_finite_field} from the computation results  $\{d^{(i)}_{jk}\}_{i,j,k\in[N]}$ by utilizing   Reed-Solomon decoding.
        % \STATE Server decodes polynomials $\{h_{jk}\}_{j,k\in[N]}$ in \eqref{eq:poly_dist} by utilizing Reed-Solomon decoder and recovers $\{\overline{d}_{jk}\}_{j,k\in[N]}$ in \eqref{eq:distance_finite_field}.
        
        \STATE Server converts $\{\overline{d}_{jk}\}_{j,k\in[N]}$ from the finite field to the real domain to obtain the pairwise distances $\{{d}_{jk}\}_{j,k\in[N]}$ from \eqref{eq:distance_real_domain}.
        
        \STATE Server selects the set $\mathcal{S}$ by utilizing the multi-Krum algorithm \cite{blanchard2017machine} based on the pairwise distances $\{{d}_{jk}\}_{j,k\in[N]}$.
        
        \STATE Server broadcasts the set $\mathcal{S}$ to all users.
    
        \FOR{user $i=1,\ldots,N$}
            \STATE Compute $\mathbf{s}_i = \sum_{j\in\mathcal{S}} \mathbf{s}_{ji}$ from \eqref{eq:SS_sum} and send the result to the server.
        \ENDFOR
        
        \STATE Server recovers $\sum_{i\in\mathcal{S}} \mathbf{w}^{(t)}_{i}$ from the computation results $\{\mathbf{s}_i\}_{i\in[N]}$ by utilizing  Reed-Solomon decoding.
        
        \STATE Server updates the global model, $\mathbf{w}^{(t+1)} = \mathbf{w}^{(t)} - \frac{\gamma^{(t)}}{q} \phi^{-1}\Big( \sum_{i\in\mathcal{S}} \overline{\mathbf{w}}_i^{(t)} \Big)$.
    \ENDFOR
%   \ENDFOR
    
    % \vspace{0.1cm}
    % \FOR{user $i=1,\ldots,N_{final}$}
    % \STATE Reconstruct the missing values in  $\{\widetilde{\mathbf{s}}_k^{(L)}\}_{k\in[N_L]}$ due to the dropped users in group $L$. 
    % \STATE Compute  $\widetilde{\mathbf{s}}_i^{(final)}$ from \eqref{eq:finalaggr} and $\bar{\mathbf{s}}_i^{(final)}$ from \eqref{eq:finalaggr_LCC}.
    
    % \STATE Send $\{\widetilde{\mathbf{s}}_i^{(final)}, \bar{\mathbf{s}}_i^{(final)}\}$ to the server. 
    % \ENDFOR

    % \EndProcedure
  \end{algorithmic}
\end{algorithm}
